Earth-Adapter: Bridge the Geospatial Domain Gaps with Mixture of Frequency Adaptation

Parameter-Efficient Fine-Tuning (PEFT) is a technique that allows us to adapt powerful Foundation Models (FMs) to diverse downstream tasks while preserving and unleashing their inherent capabilities. However, we have observed that existing PEFT methods, which are often designed with natural imagery in mind, struggle when applied to Remote Sensing (RS) scenarios. This is primarily due to their inability to handle artifact influences, a problem particularly severe in RS image features. To tackle this challenge, we introduce Earth-Adapter, the first PEFT method specifically designed for RS artifacts conquering. Earth-Adapter introduces a novel Mixture of Frequency Adaptation process that combines a Mixture of Adapter (MoA) with Discrete Fourier Transformation (DFT). By utilizing DFT, Earth-Adapter can decompose features into different frequency components, precisely separating artifacts from original features. The MoA then dynamically assigns weights to each adapter expert, allowing for the combination of features across various frequency domains. These simple-yet-effective approaches enable Earth-Adapter to more efficiently overcome the disturbances caused by artifacts than previous PEFT methods, significantly enhancing the FMs' performance on RS scenarios. Experiments on Domain Adaptation (DA), and Domain Generalization (DG) semantic segmentation benchmarks showcase the Earth-Adapter's effectiveness. Compared with baseline Rein, Earth-Adapter significantly improves 9.0% mIoU in DA and 3.1% mIoU in DG benchmarks. Our code will be released at https://github.com/VisionXLab/Earth-Adapter.

==> tables/table2.tex <==

%isaid跑的比较慢，最后再跑
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
        \toprule
         \multirow{1}{*}{Methods}  & Potsdam & Vaihingen & LoveDA & ISAID  \\
        \midrule
         Frozen & 75.6  & 70.4 & 54.2 & 67.3 \\
         Full Fine-Tune & \\
         Adapter & \\
         LoRA  & 71.9 & 64.6 & 51.0 & 48.5 \\
         VPT & 75.9   & 70.6 & 54.6 & 68.5 \\
         AdaptFormer & 65.4   & 56.0 & 42.0 & 7.5\\
         Rein & 76.2  & 70.8 & 54.9 & 68.4 \\
         Earth-Adapter (Ours) & 76.5(+0.3)  &  71.6(+0.8) & 56.0(+1.1) & -  \\
        \bottomrule
    \end{tabular}}
    \caption{\textbf{Performance Comparison of Supervised semantic segmentation on four benchmarks.} Results also demonstrate Earth-Adapter's superiority.}
    \label{tab: supervised_comparison}
\end{table}

==> tables/table_1_new.tex <==
% \begin{table*}[h]
%     \centering
%     \setlength{\tabcolsep}{0.5mm} % 设置列间距
%     \begin{tabular}{cccccccccccccccccc}
%     \toprule
%         \multirow{1}{*}{Methods}& Setting & Surf & Bldg & Vegt & Tree & Car & Clut & \multirow{1}{*}{mIoU (\%)} & Setting &Bkgd & Bldg & Road & Water & Barr & Frst & Agri  & \multirow{1}{*}{mIoU (\%)}\\
%        \midrule
%          Frozen&  \multirow{3}{*}{\parbox{1.5cm}{\centering P2V\\(DA)}}& 38.6 & 24.1 & 11.9  & 47.2 & 2.5 & 1.5 & 21.0 & \multirow{3}{*}{\parbox{1.5cm}{\centering U2R\\(DA)}} & 42.6 & 17.2 &6.7 &9.6 &0.7 & 5.7 & 0.0 & 11.8\\
%          Rein&& 75.4 & 88.6 & 50.3 & 73.4 & 59.0 &14.5 &60.2& & 27.9 &41.9&29.3 &51.2 &0.8 &\textbf{53.2} & 0.0 & 29.2
%          \\
%           \textbf{Earth-Adapter (Ours)} & &\textbf{80.3}&  \textbf{89.5 }&  \textbf{ 66.3} &  \textbf{74.4} &  \textbf{61.9 }& \textbf{33.6} &  \textbf{ 67.7} &  &  \textbf{56.3} & \textbf{ 63.4} &  \textbf{48.7} & \textbf{66.6} &  \textbf{13.7} & 38.4 & \textbf{63.2} & \textbf{50.0}\\
%           \midrule
%          Frozen&  \multirow{3}{*}{\parbox{1.5cm}{\centering P2V\\(DG)}}& 70.6 & 79.9 & 46.1  & 72.1  &\textbf{ 58.6}& 20.4 & 57.9 & \multirow{3}{*}{\parbox{1.5cm}{\centering U2R\\(DG)}} & 56.7 & 54.8 & 41.3 &\textbf{67.0} &14.6 & 15.1 & 49.2 & 42.7\\
%          Rein && 74.4 & 85.1 & 51.0 & 23.0 & 57.1  &24.5 &60.8& & 53.0 & 57.8  & 41.2 & 61.1 & 9.4  &23.4 &\textbf{57.8} & 43.4
%          \\
%           \textbf{Earth-Adapter (Ours)} & &  \textbf{76.3} &  \textbf{85.4} &  \textbf{59.0} &  \textbf{74.1} &  54.2 & \textbf{40.6}& \textbf{64.9} &  & \textbf{52.6} & \textbf{55.7} & \textbf{44.1} &  64.6 &  \textbf{17.0} & \textbf{29.6} &  56.1 & \textbf{46.7}\\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Performance Comparison of Per-Class between Frozen DINOv2-L, Rein, and Earth-Adapter on Potsdam RGB-to-Vaihingen.} Both Rein and ours are based on the Frozen DINOv2-L. The \textbf{Bold} font means the best performance.}
%     \label{tab: per-class}
% \end{table*}



% \begin{table*}[h]
% \centering
% \scriptsize % 缩小字体
% \setlength{\tabcolsep}{1mm} % 控制列间距

% % ----------------- 左侧子表格 (P2V) -----------------
% \begin{subtable}{0.48\textwidth}
% \centering
% \begin{tabular}{cccccccc}
% \toprule
% \multirow{1}{*}{Methods} & Setting & Surf & Bldg & Vegt & Tree & Car & Clut & \multirow{1}{*}{mIoU (\%)}\\
% \midrule
% Frozen & \multirow{3}{*}{\parbox{1.2cm}{\centering P2V\\(DA)}}
% & 38.6 & 24.1 & 11.9 & 47.2 & 2.5 & 1.5 & 21.0 \\
% Rein && 75.4 & 88.6 & 50.3 & 73.4 & 59.0 & 14.5 & 60.2 \\
% \textbf{Earth-Adapter (Ours)} && \textbf{80.3} & \textbf{89.5} & \textbf{66.3} & \textbf{74.4} & \textbf{61.9} & \textbf{33.6} & \textbf{67.7} \\
% \midrule
% Frozen & \multirow{3}{*}{\parbox{1.2cm}{\centering P2V\\(DG)}}
% & 70.6 & 79.9 & 46.1 & 72.1 & \textbf{58.6} & 20.4 & 57.9 \\
% Rein && 74.4 & 85.1 & 51.0 & 23.0 & 57.1 & 24.5 & 60.8 \\
% \textbf{Earth-Adapter (Ours)} && \textbf{76.3} & \textbf{85.4} & \textbf{59.0} & \textbf{74.1} & 54.2 & \textbf{40.6} & \textbf{64.9} \\
% \bottomrule
% \end{tabular}
% \caption{P2V results}
% \end{subtable}
% \hfill
% % ----------------- 右侧子表格 (U2R) -----------------
% \begin{subtable}{0.48\textwidth}
% \centering
% \begin{tabular}{ccccccccc}
% \toprule
% \multirow{1}{*}{Methods} & Setting & Bkgd & Bldg & Road & Water & Barr & Frst & Agri & \multirow{1}{*}{mIoU (\%)}\\
% \midrule
% Frozen & \multirow{3}{*}{\parbox{1.2cm}{\centering U2R\\(DA)}}
% & 42.6 & 17.2 & 6.7 & 9.6 & 0.7 & 5.7 & 0.0 & 11.8 \\
% Rein && 27.9 & 41.9 & 29.3 & 51.2 & 0.8 & \textbf{53.2} & 0.0 & 29.2 \\
% \textbf{Earth-Adapter (Ours)} && \textbf{56.3} & \textbf{63.4} & \textbf{48.7} & \textbf{66.6} & \textbf{13.7} & 38.4 & \textbf{63.2} & \textbf{50.0} \\
% \midrule
% Frozen & \multirow{3}{*}{\parbox{1.2cm}{\centering U2R\\(DG)}}
% & 56.7 & 54.8 & 41.3 & \textbf{67.0} & 14.6 & 15.1 & 49.2 & 42.7 \\
% Rein && 53.0 & 57.8 & 41.2 & 61.1 & 9.4 & 23.4 & \textbf{57.8} & 43.4 \\
% \textbf{Earth-Adapter (Ours)} && \textbf{52.6} & \textbf{55.7} & \textbf{44.1} & 64.6 & \textbf{17.0} & \textbf{29.6} & 56.1 & \textbf{46.7} \\
% \bottomrule
% \end{tabular}
% \caption{U2R results}
% \end{subtable}

% % ----------------- 总caption -----------------
% \caption{\textbf{Performance Comparison of Per-Class between Frozen DINOv2-L, Rein, and Earth-Adapter.}
% Both Rein and ours are based on the Frozen DINOv2-L. \textbf{Bold} numbers indicate the best performance.}
% \label{tab:per-class}
% \end{table*}

